Mind the Gap Between Conversations for Improved Long-Term Dialogue Generation

Knowing how to end and resume conversations over time is a natural part of communication, allowing for discussions to span weeks, months, or years. The duration of gaps between conversations dictates which topics are relevant and which questions to ask, and dialogue systems which do not explicitly model time may generate responses that are unnatural. In this work we explore the idea of making dialogue models aware of time, and present GapChat, a multi-session dialogue dataset in which the time between each session varies. While the dataset is constructed in real-time, progress on events in speakers' lives is simulated in order to create realistic dialogues occurring across a long timespan. We expose time information to the model and compare different representations of time and event progress. In human evaluation we show that time-aware models perform better in metrics that judge the relevance of the chosen topics and the information gained from the conversation.

==> Tables/auto_evaluation.tex <==
\begin{table}[t!]
    \centering
    \begin{tabular}{rc}
    \toprule
    \textbf{Model} & \textbf{Perplexity} \\
    \midrule
    MSC \cite{xu-etal-2022-beyond}       &  38.14  \\
    RAG (FT)     &  19.53 \\
    \midrule
    \textit{TA-RAG (progress)}     &   24.15 \\
    \textit{TA-RAG (schedule)}  &  24.25 \\
    \textit{TA-RAG (both)}      &  24.95 \\
    \bottomrule
    \end{tabular}
    \caption{The perplexity for the models we train.}
    \label{tab:auto_evaluation}
\end{table}

==> Tables/chatgpt_variants.tex <==
\begin{table*}[ht!]
    \centering
    \begin{tabular}{rccccc}
    \toprule
    \textbf{Model} & \multicolumn{5}{c}{\textbf{Human Ratings against RAG (FT)}} \\
    \midrule
    & Naturalness & Informativeness & Relevance & Time-Awareness & Total\\
    \midrule
    ChatGPT (progress)      & 18.08  &   \textbf{\phantom{0}5.12}  & 	15.38  &  38.78  &  19.34\\
    ChatGPT (schedule)  & 15.84  &   \phantom{0}4.54   &	12.30  &   47.78  &  20.12\\
    ChatGPT (both)      & \textbf{18.26}   &   \phantom{0}3.80  &   \textbf{ 17.30}  &  \textbf{52.58}  &  \textbf{22.99} \\
    \bottomrule
    \end{tabular}
    \caption{Time errors made by models fine-tuned on different datasets.}
    \label{tab:chatgpt_variants}
\end{table*}

==> Tables/estimate_duration.tex <==
\begin{table}[bh!]
    \centering
    \begin{tabular}{l}
    \toprule
    \textit{Prompt} \\
    \midrule
    Each event takes certain time to finish. For \\ 
    instance, writing a conference paper takes \\
    around 3 months, watching a movie takes around \\
    2 hours, having lunch takes around 1 hour, \\
    having a vocation to the beach takes around 1 \\
    week, finishing a master program takes around 2\\
    years. For the events listed below, give an \\
    estimation of the time to finish. \\
    working on their doctorate thesis takes about \_\_\_. \\
    participating in a book reading event takes \\
    about \_\_\_. \\
    Fill in the blanks with the amount of time. \\
    \midrule
    \textit{Result} \\
    \midrule
    around 3 years \\
    around 2 hours \\
    \bottomrule
    \end{tabular}
    \caption{Prompt to estimate duration of extracted events.}
    \label{tab:estimate_duration}
\end{table}

==> Tables/extract_events_prompt.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l}
    \toprule
    \textit{Prompt} \\
    \midrule
    In the following conversation, speaker 1 and \\
    speaker 2 are updating their daily lives. In \\
    the conversation, both speakers might have \\
    mentioned some events they are engaging. \\
    Summarize these events and fill in the blanks. \\
    Speaker 1: Hi, how are you doing? \\
    Speaker 2: Hi, I’m doing great, how about \\
    you? \\
    Speaker 1: I’m also doing good. How is\\
    everything?  \\
    Speaker 2: I'm good. I'm just busy with my \\
    doctorate thesis. It's tough, but I could make\\
    some progress on the literature review. \\
    ...\\
    In this conversation, speaker 1 is engaging in\\
    \_\_\_ and speaker 2 is engaging in \_\_\_. \\
    \midrule
    \textit{Result} \\
    \midrule
    Speaker 1: preparing for exams. \\
    Speaker 2: working on their doctorate thesis, \\
    participating in a book reading event.\\
    \bottomrule
    \end{tabular}
    \caption{The prompt to extract the events of speakers.}
    \label{tab:extract_events}
\end{table}

==> Tables/fine_tune.tex <==
\begin{table*}[ht!]
    \centering
    \begin{tabular}{rcccccccc}
    \toprule
    \textbf{Model} & \multicolumn{2}{c}{Vanilla} & \multicolumn{2}{c}{MSC only} & \multicolumn{2}{c}{EventChat only} & \multicolumn{2}{c}{MSC-EventChat} \\
    \midrule
    & F-1 & PPL & F-1 & PPL & F-1 & PPL & F-1 & PPL \\
    \midrule
    MSC               &   &   & - & - &   &   &   &    \\
    MSC-RAG           &   &   & - & - &   &   & - & -  \\
    SumMem-MSC RAG    &   &   & - & - &   &   & - & -  \\
    \bottomrule
    \end{tabular}
    \caption{Performance of different models in \textit{perplexity} when fine-tuned on EventChat.}
    \label{tab:fine_tuning}
\end{table*}

==> Tables/no_annotation.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{ccccc}
    \toprule
    \textbf{Model} & \multicolumn{4}{c}{\textbf{Ratio of Conversations with Time Errors}} \\
    \midrule
                    &  Vanilla & MSC only & EventChat only & MSC-EventChat \\
    \midrule
    BST 2.7B        &          &          &                &          \\
    MSC 2.7B        &          &          &                &          \\
    MSC-RAG 2.7B    &          &          &                &          \\
    MSC-FiDRAG 2.7B &          &          &                &          \\
    \bottomrule
    \end{tabular}
    \caption{Time errors made by models fine-tuned on different datasets.}
    \label{tab:time_errors}
\end{table*}

==> Tables/prompt.tex <==
\begin{table}[ht!]
    \centering
    \begin{tabular}{l}
    \toprule
    \textit{Task description} \\
    \midrule
    Extract events in the following conversation. \\
    An event is an action or social activity that \\
    needs to be finished in a period of time. \\
    \midrule
    \textit{Instances $*N$} \\
    \midrule
    Dialogue: \\
    A: Hi how are you? \\
    B: Yes I am fine and how are you doing today? \\
    A: Doing good. What is the plan for to night? \\
    B: Not yet planed for something. I just started \\ 
    with preparing and executing a social media \\ 
    marketing campaign for my company. \\
    A: Oh are you busy in that? \\
    B: Yes it takes 3 months to finish the work. \\
    Events: \\
    preparing and executing a social media \\ 
    marketing campaign. \\
    \midrule
    \textit{Question dialogue} \\
    \midrule
    Dialogue: \\
    A: Hi, how are you doing? \\
    B: I'm doing great, how about you? \\
    A: I'm also doing good. I'm just busy with my\\
    paper writing as the deadline is approaching. \\
    Events: \\
    \bottomrule
    \end{tabular}
    \caption{The prompts we use to extract events from existing dialogue history.}
    \label{tab:prompt}
\end{table}

==> Tables/time_aware_variants.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{rc}
    \toprule
    Model & PPL \\
    \midrule
    Time-aware RAG (no summaries) &  \\
    Time-aware RAG (dialogue segments) & \\
    Time-aware RAG (with schedules) & \\
    \midrule
    Time-aware RAG  & \\
    \bottomrule
    \end{tabular}
    \caption{The Perplexity of time-aware RAG model with different information as inputs for the dialogue generation.}
    \label{tab:model_variants}
\end{table}

==> Tables/time_error.tex <==
\begin{table*}[ht!]
    \centering
    \begin{tabular}{ccccc}
    \toprule
    \textbf{Model} & \multicolumn{4}{c}{\textbf{Ratio of Conversations with Time Errors}} \\
    \midrule
                    &  Vanilla & MSC only & EventChat only & MSC-EventChat \\
    \midrule
    \textit{With time annotations} \\
    \midrule
    BST 2.7B        &          &          &                &          \\
    MSC 2.7B        &          &          &                &          \\
    MSC-RAG 2.7B    &          &          &                &          \\
    MSC-FiDRAG 2.7B &          &          &                &          \\
    \midrule
    \textit{Without time annotations} \\
    \midrule
    BST 2.7B        &          &          &                &          \\
    MSC 2.7B        &          &          &                &          \\
    MSC-RAG 2.7B    &          &          &                &          \\
    MSC-FiDRAG 2.7B &          &          &                &          \\
    \bottomrule
    \end{tabular}
    \caption{Time errors made by models fine-tuned on different datasets.}
    \label{tab:time_errors}
\end{table*}

==> trash/data.tex <==
% ======================= Qiang ============================== %
% Although the time gaps between sessions were marked in MSC, such a time feature was not completely embedded into the conversations, which led to the conclusion that the time feature has only minimal effect on the models' performance~\cite{xu-etal-2022-beyond}. 
% The reason is that speakers are not instructed to have conversations with respect to the temporal relationship between the duration of the events and the session time gaps.


% We follow the general settings in MSC and collect a conversation dataset, \dataset{}, through Amazon Mechanical Turk. 
% Unlike MSC, where speakers have aimless and meaningless free chitchats without concentrating on specific topics, speakers in \dataset{} are having conversations in a simulated world where speakers follow their unique life timelines in a time range. 
% The speakers are required to talk about their timelines, which contain the progress of ongoing events depending on the time gap between sessions. 
% Another difference between \dataset{} and MSC is that speakers are different for each session in MSC. 
% However, to better simulate the long-term relationship between speakers, we collect multi-session dialogues from the same speakers in \dataset{}.

% ======================= ChatGPT ============================== %
% ======================= Qiang ============================== %
% We use \textit{Timelines} to simulate the speakers' lives as if they are having conversations based on their experiences in the real world.  
% As shown in Figure~\ref{fig:timeline}, each \textit{Timeline} consists of one or many events a speaker has finished depending on the events' schedules and the conversation's time span. 
% We pre-define events and their schedules, ranging from 3 hours to 1 year. Speakers are asked to stick to the current schedule and engage in conversations to update their ongoing events concerning the time gaps between sessions. 
% There are three types of events defined in \dataset{}: \textbf{progress events}, \textbf{life events}, and \textbf{world events}. Examples of each type of event can be found in Appendix A.

% ======================= ChatGPT ============================== %
% ======================= Qiang ============================== %
% A progress event is an event that needs to be finished following a particular schedule. 
% For instance, the event of ``attending a 3-day basic cookery course'' requires about 1 day to finish the introduction, 1 day to learn knife skills and 2 days to learn to cook basic dishes. 
% Progress events provide the continuity of the context in a multi-session conversation. 
% As time moves forward, there will be new progress in these events, and speakers are instructed to have conversations based on the progress. 
% By estimating the duration of events and the gaps between sessions, speakers may behave differently regarding the progress (e.g., avoid talking about events that take a long time when the session gap is short). 
% In this way, we capture how humans converse based on when they are asked to express their perception of time.

% ======================= ChatGPT ============================== %
% ======================= Qiang ============================== %
% \paragraph{Life Events}
% Life events are events that take a relatively short time to finish when compared to ongoing progress events. 
% For instance, ``visiting a museum'', which takes about 2 days, is a life event compared to ``learning Spanish'', which usually takes years. 
% We use life events to simulate the sudden external information that happens to them and enrich the topics to talk about when there is no significant progress on the progress events. 

% \paragraph{World Events}
% A world event is usually a piece of news that is happening around the world (e.g., ``Argentina won the championship of World Cup.'') 
% The key point of a world event is that it should be acknowledged by both speakers in the conversation so that the speakers can easily extend a discussion. 
% In this way, speakers can feel more sense of the real world.

% ======================= ChatGPT ============================== %
% ======================= Qiang ============================== %
% Sessions in MSC contain 12-14 utterances, which makes it difficult for the speakers to develop deep discussions before they switch to a new session. 
% Therefore, in the new session, regardless of the time gap, speakers frequently continue the conversation immediately, which is unnatural. 
% In \dataset{}, we extend each session to at least 20 utterances and require each session to start and end naturally (e.g., greetings, closures). 
% Moreover, speakers are instructed to pay close attention to the time gap between sessions, which might affect how they would behave in the new session.

% ======================= ChatGPT ============================== %
% ======================= Qiang ============================== %
% When the session length reaches the minimum requirements, and either speaker wants to end the current session, the speakers can move the time forward and create a time gap of a random period of time for a new session, ranging from 10 minutes to 1 year. At the same time, the speakers are provided with the progress of the events according to the schedules and the time gap. If the time gap is shorter than the minimum necessary time to reach the next step in the schedule, speakers will be provided a message of ``No significant progress.'' And if the time gap covers the full duration of the event, speakers will be provided a message of ``You finished the previous event. And <new progress event>'' and assigned a new progress event. Each time when the time moves forward, the speakers are also provided with randomly selected life events and world events. They could choose either to talk about such events or to ignore them. The conversations in \dataset{} contain 3-7 sessions.
% Samples of conversations consisting of different numbers of sessions can be found in Appendix B.

% ======================= ChatGPT ============================== %

==> trash/intro.tex <==
% =============================
% Questions to answer:
% 1. What is the problem you're going to solve?
% 2. Why is this problem serious?
% 3. What are the existing solutions to this problem?
% 4. What is your solution and why is it different?
% 5. Your contributions
% =============================

% ACL Policy on AI Writing Assistance
% https://2023.aclweb.org/blog/ACL-2023-policy/

% ======================= Qiang ============================== %
% The perception of time is fundamental in human awareness~\cite{di2018feel}. 
% Yet, surprisingly, the effectiveness of perception of time when building dialogue systems is still unknown. 
% In daily conversations, humans frequently ``update news'' to track ongoing events in the interlocutors' lives to maintain closeness~\cite{bolden2006little}. 
% This requires a model to have the perception of time to judge the current status of ongoing events to generate natural and appropriate responses. ~\cite{bolden2006little} 

% ======================= ChatGPT ============================== %
% The awareness of time is a crucial aspect of human perception~\cite{di2018feel}. 
% Despite its significance, the extent to which time perception contributes to the efficacy of dialogue systems remains uncertain. Human communication involves regular updates on current events in the lives of the interlocutors as a means of nurturing intimacy~\cite{bolden2006little}. 
% This necessitates the integration of time perception into the system to enable an accurate assessment of the ongoing events and generate contextually appropriate and natural responses.

% core: the systems generate frustrating questions

% ======================= Qiang ============================== %
% According to the pragmatic theory by Grice~\cite{grice1975logic,grice1989studies}, humans expect to have effective and informative conversations. As shown in Figure~\ref{fig:intro}, the speaker might not want to be asked about the progress of the thesis in only 2 hours. The reason is that humans acknowledge that writing a doctorate thesis takes years and one will not make significant progress in only several hours. And asking the progress of a long-term event in a short interval makes the conversation less effective and cooperative. Instead, the speaker expect to exchange information on events of which the status could have changed during the time gap or talk about the progress of writing the thesis after a longer time gap (e.g., two weeks) in order to have natural and effective conversations.

% ======================= ChatGPT ============================== %
% Drawing from Grice's pragmatic theory~\cite{grice1975logic,grice1989studies}, human conversational exchanges are typically expected to be informative and effective. 
% As depicted in Figure~\ref{fig:intro}, a speaker may not desire to be questioned about the status of their doctoral thesis within a brief two-hour timeframe. 
% This is primarily due to the understanding that such an academic pursuit takes several years, rendering any significant progress unlikely within such a limited period. 
% Consequently, posing such questions regarding the progress of a long-term endeavor in a short interval has the potential to undermine the effectiveness and cooperation of the conversation.
% Instead, the speaker expects a conversation that focuses on events whose status may have changed during the time lapse, or a discussion regarding the progress of the thesis after a more extended duration, such as two weeks, to have a more natural and productive conversation.

% The perception of time is a fundamental aspect of human cognition (Di Russo, et al., 2018). Effective communication depends on one's ability to update information without asking irrelevant and frustrating questions that can harm social bonds (Bolden, 2006).

% ======================= Qiang ============================== %
% Existing long-term dialogue models have more or less considered the perception of time. 
% For instance, ~\citeauthor{xu-etal-2022-beyond} (\citeyear{xu-etal-2022-beyond}) released the Multi-Session Chat (MSC) dataset, in which the time gaps between sessions are marked. 
% However, we consider three issues in MSC. 
% First, MSC does not simulate the ``lives'' of the speakers in a way that they should focus on the ongoing events in a period of time, which is one of the most important parts of real-world human lives. As a result, conversations in MSC are aimless and more time-irrelevant.
% Second, sessions in MSC are too short for speakers to develop natural dialogues that include greetings and closures. 
% Moreover, speakers are not clearly instructed to pay attention to the time gap. 
% Therefore, speakers tend to continue the topics in a new session, regardless of the time gap. 
% Third, each session in MSC is generated by different speakers, which could significantly break the continuity among consecutive sessions. 
% New speakers frequently lose interest in the previously mentioned topics and give up tracking the status of previous events.
% These issues eventually led to the conclusion in MSC that the time gap only has a minor effect on the performance of the models.
 
% ======================= ChatGPT ============================== %
% Some long-term dialogue models have considered the perception of time.
% For instance, ~\citeauthor{xu-etal-2022-beyond} (\citeyear{xu-etal-2022-beyond}) introduced the Multi-Session Chat (MSC) dataset, which features time intervals between sessions. 
% Nevertheless, we identify three critical shortcomings in MSC. First, the dataset fails to capture the speakers' ``lives'' accurately, which entails monitoring ongoing events over a certain period, an essential component of real-life conversations. 
% Consequently, conversations within MSC appear directionless and lack temporal relevance. 
% Second, the session duration in MSC is too brief for speakers to establish natural dialogues that include salutations and conclusions. 
% Furthermore, the dataset does not provide explicit guidance to the speakers regarding the time interval, leading them to continue previous discussions even after prolonged breaks. 
% Third, different speakers generate each session within MSC, causing a disruption in the continuity of the dialogue. 
% As a result, new speakers frequently lose interest in prior topics, thereby hindering the ability to track the status of previous events. 
% These limitations have resulted in the conclusion that the impact of time gaps on the models' performance is insignificant within the MSC dataset.

% ======================= Qiang ============================== %
% In this work, we study a way to simulate the ``lives'' of interlocutors so that they focus on conversing about ongoing events with respect to the duration of the events and the time gaps between sessions.
% To do that, we first collect a multi-session dialogue dataset called EventChat following the MSC dataset. 
% We design simulated timelines for speakers, which simulate the events and associated schedules that the speakers will engage in a period of time during the conversations. Speakers are then asked to have natural conversations while sharing the progress of ongoing events following the simulated timelines.
% Sessions in our dataset are longer and more naturally connected through the status of events.    
% Moreover, we invite the same speakers throughout all sessions in the conversations to maintain better continuity.
% Dialogue models are trained on this dataset to learn the representations of events' status as time passes. 
% And at inference time, we use the large-scale language model LLaMA~\cite{touvron2023llama} to automatically generate schedules and necessary temporal information, including the duration of ongoing events and the time gap between sessions through prompting~\cite{brown2020language}. 
% Different prompts are attempted to explore the effectiveness. Finally, together with the user inputs, prompted time information is fed to the dialogue model to generate responses.

% The contributions of this work are as follows:
% \begin{itemize}
%     \item We design and implement simulated timelines for collecting conversations in which speakers' perception of time is required to produce natural communications. 
%     \item We collect a multi-session conversation dataset, which highlights the speakers' perception of time during communication.
%     \item We show an overall improvement in the naturalness of the dialogues generated by a variety of dialogue models that are fine-tuned on our dataset.
% \end{itemize}

% In this study, we aim at building time-aware dialogue models that enhance the naturalness of the conversations in terms of maximizing the information gain. 
% We do this with our newly collected dataset~\dataset{}, which extends the MSC dataset. 
% Unlike in MSC, where speakers do free chit-chats based on a set of unrelated personas, speakers in~\dataset{} have conversations based based on simulated timelines. 
% These timelines are carefully designed to simulate the speakers' ``lives'', reflecting their engagement in various events during the conversation period. 
% Speakers are instructed to have natural conversations while reporting on the progress of the ongoing events with respect to their timelines. 
% Compared to MSC, our dataset also features longer sessions that are naturally connected by the status of the events and involves the same speakers throughout to enhance continuity.
% We then construct the time-aware dialogue model on this dataset by retrieving necessary time related information such as duration of the events, possible schedules of the events from possible knowledge sources. The experiments show that by providing time information, our time-aware model is able to have conversations in a way that human evaluated as more natural, informative and relevant.

% The contributions of this study include: (1) the creation of a multi-session conversation dataset that emphasizes speakers' perception of time during communication, (2) the exploration of different ways to model time and construct time-aware dialogue models, and (3) the evaluations of the models that focus on maximizing the information gain in the conversations.

% ======================= ChatGPT ============================== %

% In this study, we aim to simulate the temporal awareness of speakers during conversations by focusing on ongoing events and their respective durations, as well as the time gaps between sessions. To achieve this, we introduce~\dataset{}, a multi-session dialogue dataset that extends the MSC dataset.~\dataset{} includes simulated timelines for each speaker, reflecting their engagement in various events during the conversation period. The speakers are then asked to engage in natural conversations while reporting on the progress of the ongoing events based on the simulated timelines. Compared to MSC, our dataset features longer sessions that are naturally connected by the status of the events and involves the same speakers throughout to enhance continuity. We then train various dialogue models on the dataset to learn representations of the events' status over time, and at inference time, we use LLaMA~\cite{touvron2023llama}, a large-scale language model, to automatically generate schedules and temporal information (e.g., the duration of ongoing events) via prompting. We try various prompts to explore the effectiveness of different prompts. And the prompted time information is fed to the dialogue models along with user inputs to generate responses.

% The contributions of this study include: (1) the introduction of simulated timelines for collecting conversations that require speakers' temporal awareness to generate natural communication, (2) the creation of a multi-session conversation dataset that emphasizes speakers' perception of time during communication, and (3) the demonstration of the overall improvement in the naturalness of the dialogues generated by various fine-tuned dialogue models on our dataset.

% This requires the models to judge the status of current ongoing event based on the understanding of time.

% However, in daily conversations, human beings periodically ``update news'' to track ongoing events in the interlocutors' lives to maintain closeness~\cite{bolden2006little}. 

% Human beings periodically ``update news'' to track ongoing events in the interlocutors' lives to maintain closeness~\cite{bolden2006little}. This becomes important when building open-domain dialogue system to have long-term conversations. Commonly used method is to load 
% However, one issue that has been ignored by current long-term open-domain dialogue models is that humans judge the status of current ongoing event based on the understanding of time, whereas the current systems suffer in this setting. 


% Understanding time is essential in human daily conversations, in which 

% With improvements in large-scale language models, building long-term open-domain dialogue systems draws a lot of attention~\cite{xu-etal-2022-beyond,xu-etal-2022-long,zhang2023history}.

% Open-domain dialogue systems are supposed to have long-term conversations to maintain a long-term relationship with the users while being able to converse on any topics and events~\cite{clark2019makes,roller-etal-2021-recipes,zhang2023history}. Benefit from large-scale pre-trained language models, existing dialogue systems are able to load and encode a longer dialogue history to generate history-based responses with a certain level of consistency.

% As time accumulates, more and more topics and events are involved in the conversation. How to select the best topics for future communications becomes a challenging task when building long-term open-domain dialogue systems.    Existing solution of simply loading and encoding the complete dialogue history as in~\cite{xu-etal-2022-beyond,xu-etal-2022-long,zhang2023history}, treats all topics and events equally and fails to highlight the most urgent topics. As a result it is easy for such models to generate responses that are not appropriate to be mentioned at current timing.



% Existing solution simply loads and encodes a longer dialogue history to generate history-based responses with certain level of consistency, whereas it fails to 

% Benefit from large-scale pre-trained language models, existing dialogue systems are able to load and encode a longer dialogue history to generate history-based responses with a certain level of consistency.

% Although loading a longer history helps when , it fails to highlight the 

% Existing intuitive solutions simply load previous dialogue history into the model to generate response based on longer context, however ignoring the continuity of the events in the conversation. The sessions in such conversations have very limited connections and talk about totally different events and thus can hardly be treated as one long-term conversations. Additionally, time duration between each session can be an important indicator for topic selection. However, previous works selectively ignore this, which can makes the conversations factually-conflicting (e.g., report a big progress of a long-term task in a very short time).

% Rather than topic-free conversations, we collect multi-session conversations where the sessions connect to each other tightly through pre-defined schedules. We collect sessions that contain consistent topics as defined in the schedules and reflect the time duration.

% Long-term conversations use multiple dialogue sessions to progress a long-term goal.
% The time that has elapsed since the previous session affects the strategies used in further sessions.   In particular, the progress of a long-term goal (e.g., dissertation writing, medical treatment, etc.) is probably not mentioned in two consecutive sessions with an interval of several minutes. And a short-term goal (e.g., cooking dinner, taking a shower, etc.) that had been mentioned in a previous session years ago should not be brought back in a new session. 
% Existing works on multi-session chat either simply loads the previous dialogue history or pass the information through summaries~\cite{xu-etal-2022-beyond}, which does not explicitly model the time effect and can lead to inappropriate responses. 
% For instance, we observe that existing memory enhanced Blenderbot model~\cite{roller-etal-2021-recipes} asks ``\textit{How is your dissertation going on?}'' in a new session that is only several hours after the previous session discussing the progress of the dissertation, which is a long-term goal that takes years to finish and can hardly be significantly progressed in several hours.    One reason is that such models do not have the ability to clearly understand the time effect of the events (what is an event, need a definition here, or some references?) in the conversations, though they are able to generate responses on the same topic. 

% This work focuses on modeling the time effect in multi-session conversations and shows how such time-aware models can generate better responses in terms of reengaging/resuming incomplete conversations. We collect and release a time-augmented multi-session conversation dataset that contains human-human goal-oriented discussions over multiple sessions on 5 topics of A, B, C, D and E. For each new session, we assign a certain amount of time that has elapsed since the previous session and require crowdworkers to generate new sessions with respect to the goal, topic and time of the discussion.  The dataset features time annotations of the events that have been mentioned in the previous sessions to hint the strategies for mentioning them in future sessions. When performing new sessions, the crowdworkers are provided both the dialogue history of previous sessions and time annotations of the events to either pursue deep discussions on the previous topics or raise new topics with respect to the time that has elapsed since the previous session. 

% We first examine the performance state-of-the-art FiD-RAG model~\cite{xu-etal-2022-beyond} on our collected dataset and show it has difficulty distinguishing the time effect of events even with fine-tuning. The results show that existing models have no ability to extract or understand the time effect even with human annotations. To address this issue, a new RAG model with reasoning ability is proposed where we use pre-trained language models to extract the time effect.

% \paragraph{method}
% In the work, we follow the Ask an Expert method and utilize pre-trained language models to provide necessary knowledge on the time effect of activities in the dialogue history.   More specifically, we first extract the activities in previous sessions which could be possibly mentioned for a new session and prompt language models the time duration of such activities.   Dialogue models then learn the representations of such time duration and generation time-aware responses in new sessions. 

% \paragraph{Multi-session Chat}
% There is not many existing datasets on multi-session conversations. To the best of our knowledge, the only previous work is the Multi-Session Chat (MSC)~\cite{xu-etal-2022-beyond}. In MSC, crowdsource workers are asked to play roles with certain personas and have multi-session conversations with random time duration among sessions. To reduce the total length of the text each worker must read, MSC features a human annotated summary for each session which is much shorter than the dialogue history. MSC allows speakers to resume the conversation and reengage the events in previous sessions, but it has two main disadvantages. First, it does not model the expected duration of activities which causes inappropriate utterances (after a five minute pause, asking the participant if they’ve made significant progress on their dissertation from the time of the preceding conversation). Second, the task of chatting freely means that there is little incentive for later sessions to revisit ideas of previous sessions, leaving sessions largely independent of one another and failing to distinguish the task from typical dialogue tasks.  In contrast, our work asks speakers to make references to the duration of activities in previous sessions and define a goal at the beginning of conversations. 

% \paragraph{Models for Multi-session Conversation}
% One approach for multi-session conversation is to model the dialogue using encoder-decoder Transformer based large language models. This approach has a simple implementation, where the model accesses previous sessions by directly concatenating the dialogue history as part of the input to the encoder. This method takes less effort to build the models, but it suffers from the limited input length of the encoder-decoder models (tokens in multi-session dialogues can be several thousand and the limit for existing models are mostly less than 1k). Another approach to solving that issue is Retrieval-Augmented Generation (RAG). Instead of loading the complete dialogue history of previous sessions, RAG uses a retrieval system that selects only part of the dialogue history to be included in the encoding process. An alternative version of this approach is to add additional annotations on the text to retrieve from, rather than the dialogue history only (as was done in ~\cite{xu-etal-2022-beyond} by adding summaries to each previous session). Our work follows this approach, but we focus on annotating the duration of activities in the previous sessions.

% MSC uses simulated time duration.
% MSC uses different speakers for different sessions of a conversation.
% MSC does not bridge the sessions.

% The purpose of data collection is to collect conversations in which the participants explicitly understand the conflicts between the duration of certain events and the session gaps so that participants avoid talking about these events until an appropriate gap has passed. To do that, we follow the data collection paradigm in MSC with two main modifications. First, instead of picking random participants for each session in the same conversation, we ask the same participants to finish all the sessions.   Second, during the session gaps, we provide updates (e.g., ongoing event progress, news) to the character they are playing.

% Two participants are each assigned a character they will play in the conversation.   A character is defined as a set of short sentences describing personalities and attributes.   GPT-3 is used to generate a variety of characters automatically through prompting.    Participants are asked to have free multiple sessions of chit-chat while keeping the consistency in their characters. Before each new session, we decide a time gap between the new session and the previous session. The events and activities mentioned in each previous session are extracted with a PLM-based extractor. GPT -3 is used to automatically generate updates on these events and activities based on the time gap.    The participants are provided with the updates and the time gap before starting a new session.    To collect richer content in the conversation, we also add random updates irrelevant to the conversation (e.g., ongoing news). The participants can choose anything they want to discuss in the new session.

% We collect the Time-Aware Multi-session Conversations (TAMC) to support research on the influence of activity duration in long-term conversations with inspirations from the MSC dataset. 
% We improved the original data collection procedures of MSC to allow the formulation of the duration of activities in each session, as shown in Figure~xxx.

% First, the time in MSC is simulated, which means that the time in the dataset is not the time that has passed in the real world (e.g., 8 hours in the dataset might be several minutes in the real world, which depends on how fast the crowdsource workers pick up the task). 
% Such a setting affected the quality of a new session whose previous session happened a long time ago and ended with a short activity. 
% That is, the speakers in the new session tend to directly continue to talk about the short activity even though a long time should be considered to have passed by the speakers.   
% To address this issue, we use the real-world time between sessions. 
% The time in our setting ranges from several hours to one week to create a sense of time flow.

% Second, workers of the sessions in one conversation might be different people in the original collection procedures. This creates gaps in writing style in different sessions and thus introduces meaningless biases. To avoid such biases, we pair the same workers to finish all the conversation sessions, which helps our collected conversations have more consistent writing styles.

% Third, we have noticed that it is difficult for the workers to develop a new session based on only the dialogue history of previous sessions because the workers cannot be so creative in making new episodic stories. 
% Therefore, in our setting, before a new session, the speakers are provided manually authored updates, which are stories based on the activities they discussed in previous sessions. 
% The speaker can then try creating new episodes or sharing the updates.

% \paragraph{Long-term Goal}
% We set a long-term goal for both speakers at the beginning of the conversation to keep all sessions densely connected rather than inconsistent, as in MSC. Speakers are instructed to pursue their long-term goals in all sessions instead of having meaningless free chitchats. 
% In this work, we design 5 long-term goals, including finishing the Ph.D. course, receiving psychological treatment, xxxx, yyyyyy, and zzzzzz. The time that is need for reaching these goals in the real world ranges from several days to several years and thus helps to create a balanced dataset.

% \paragraph{Initial Session}
% We collect the initial sessions with the personas from the PERSONACHAT dataset~\cite{zhang-etal-2018-personalizing}. 
% These personas are short sentences describing characteristics of the roles that the speakers are playing, which can contribute to the higher content diversity of the final dataset.
% Unlike MSC, in which the first sessions are conversations directly taken from the PERSONACHAT dataset, we only utilize the personas and collect conversations from real human speakers. 

% We randomly pick 5 out of 1,155 personas for each speaker in a conversation and assign a randomly picked long-term goal for them. The speakers then talk for up to 7 turns for an initial session. 

% \paragraph{Subsequent Sessions}
% After a random amount of time has elapsed since the previous session in the real world, we ask the same speakers to continue the conversations and develop the conversations towards their unfinished long-term goal. The time break between sessions in the real world ranges from several hours to one day, considering the time cost in the real world. To distinguish from the assumed time duration between sessions, we call this real-world time break ``real-world duration'' and the assumed time duration ``in-session duration''.
% We collect 1000 episodes with 3 sessions and 500 with 4 sessions.

% \paragraph{Episodic Updates}
% During the real-world duration between two consecutive sessions, we run another independent task to collect ``what could have happened (in the in-session duration)'' for each speaker based on what has been said in the previous sessions, denoted as episodic updates. 
% For instance, if one speaker has mentioned his/her service in the army in previous sessions and the in-session duration is 3 months, a possible episodic update for that speaker could be: \\

% \noindent ``\textit{In these 3 months, you participated in 3 different special military actions and got your left shoulder hit by a bullet.}'' \\

% The episodic updates will then be provided together with the previous sessions to the speakers so that they have more content to talk about while trying to reach their long-term goal, rather than doing meaningless chitchats, as in MSC.   We collect the episodic updates using two methods: prompting large-scale pre-trained language models and crowdsourcing.  

% Recent works show that pre-trained language models have the ability to generate creative stories and events through few-shot prompting, which can be utilized to collect episodic updates quickly. 
% We formulate the task of collecting episodic updates as a text generation task, where the language models take a given conversation between two speakers with the in-session duration as input and output text describing the possible updates for both speakers. 
% Figure xxx shows an example of prompting the language models, and the green part is the generated episodic updates.

% Although it takes less effort to collect the episodic updates through prompting language models, it might still fail to generate sense-making stories.   Therefore, it is necessary also to collect episodic updates by human annotators. Such human-annotated data can also serve as baselines when exploring the extent to which different models can perform the episodic updates generation task.

% We collect the human-annotated episodic updates with a separate crowdsourcing task, where the workers are given the dialogues of previous sessions and the in-session duration to develop stories for each speaker.   
% The stories must be feasible to happen within the in-session duration based on the context provided in the dialogue history.  We encourage the workers to generate their own versions of stories as much as possible to increase the diversity of the dataset.   

% In the later process of collecting subsequent sessions, we provide episodic updates generated by both the models and human annotators, and ask the speaker to choose the updates that they prefer to use in a new session. 

% \section{Time-Aware Modeling}

% We first extract the events and activities from the dialogue history.   PLMs are utilized to perform reasoning on time spans of these events and the duration between sessions following the method of Ask an Expert.  Such reasoning then instructs a retrieval-augmentation generation (RAG) model to generate time-aware responses.  

% \subsection{Extracting Events and Activities}
% The events and activities are extracted by an automatic event extraction model. 


% \subsection{Event Time Reasoning by PLM}

% We prompt large-scale language models, GPT-2 and GPT-3 to retrieve the time spans of the extracted events.


% need to raise the importance of time. that's how it can be called time-aware.
% this is not imporant for the story, what's the meaning of putting this sentence?
% what's the connection between training large-scale and encoding longer history? These are two things.
% getting to the point but the claim becomes very weak.

% This requires the model to be not only contextual but also time-aware to judge the status of current ongoing events correctly. As shown in Figure~\ref{fig:intro}, imagine a multi-session conversation where speakers A and B discuss the progress of speaker A's doctorate thesis in the first session, which usually takes years to finish. The speakers will likely not talk about the progress of the thesis again in a following-up session that is only around 30 minutes after the previous one. The reason is that humans commonly acknowledge that one will not make significant progress on a doctorate thesis in 30 minutes, even though this event (writing thesis) is frequently mentioned in the previous dialogue history. Such perception of time is important for predicting the progress of the ongoing events when choosing appropriate conversation topics to show warmth~\cite{roy2021enhancing} and improve user experience~\cite{dong2014time}, which are essential when building open-domain dialogue systems~\cite{de2005assessing}.

% As shown in Figure~\ref{fig:intro}, imagine a multi-session conversation where speakers A and B discuss the progress of speaker A's doctorate thesis in the first session, which usually takes years to finish. 
% The speakers will likely not talk about the progress of the thesis again in a following-up session that is only around 30 minutes after the previous one. 
% The reason is that humans commonly have the perception of time and acknowledge that one will not make significant progress on a doctorate thesis in 30 minutes. If B had fully processed and remembered the information from the first session, they would be able to judge the status of the event ``writing a doctorate thesis''. Therefore, asking about the progress of the thesis again so soon after the first session might indicate that B was not fully engaged in the conversation at the time. Avoiding such errors is important to secure effective communication and mutual understanding.

==> trash/modeling_time.tex <==
% \subsection{Time Aware Information}
% Adding explicit time information such as sessions gaps, event duration may help the model have a better sense of the time passage. We explore a method of saving such time information into the documents of the RAG model by concatenating such information with the session summaries.

% \paragraph{Session gaps only}
% Session gaps are randomly generated periods of time ranging from 10 minutes to 1 year in the format of natural language text (e.g., 1 week, 2 months). 

% \paragraph{Duration of the events}
% The model might be able to be time-aware by directly compare the sessions gaps and the duration of the events.  The duration of a event is the time length to finish that event in the format of natural language text (e.g., taking a basic cookery course: about 5 days), which is given in the pre-defined schedules. We concatenate the duration of ongoing events with the summaries and gaps.

% \paragraph{Finished progress}
% The progress of ongoing events can be determined by comparing pre-defined schedules of events to the elapsed time since the beginning of the conversation. 
% For example, if we consider the schedule for "writing a thesis," it may consist of seven steps, where the second step requires the literature review of related works to be finished by the end of the third month, and the third step requires the completion of experiment setup by the end of the fifth month. 
% If four months have passed since the beginning of the conversation, the current progress would be 28.6\% (2/7). 
% To incorporate this progress information into the dialogue system, we concatenate both the percentage progress and the text of all completed steps with the session summaries and gaps.

% \paragraph{Unfinished future progress}
% It has been observed that speakers may discuss future steps of ongoing events to facilitate more detailed conversation. It is therefore worthwhile to investigate how such information may influence the behavior of dialogue models.
% Similar to the method of adding progress information, we concatenate the full schedule of the events, which also include unfinished steps with the summaries and session gaps. 

% \paragraph{Event related dialogue segments}
% Dialogue history might be necessary for a model to capture time references aside for the summaries. But storing the entire dialogue history results in large amount of context to retrieve from~\cite{xu-etal-2022-beyond}. We use a dialogue topic segmentation model~\cite{xing-carenini-2021-improving} to segment the dialogue history and select only segments that are related to the ongoing events. This way, we can retain more dialogue information while minimizing the content.

% \paragraph{Sequence of actions}
% Schedules of events might be reflected as a sequence of actions.

% \subsection{Knowledge Base for Time Information}
% During training time, we use the pre-defined schedules described in Section~\ref{sec:timelines} as knowledge base. However, this is unrealistic during inference time as the events in the user utterances can be not in the pre-defined schedules. Therefore, we try two different types of knowledge bases.

% \paragraph{Large-scale Language Models}
% Large-scale language models (LLMs) have the knowledge about duration of time and could potentially generate schedules of the events. 
% In our experiments, we explore another method using LLMs such as LLaMA~\cite{touvron2023llama} to extract events and time information through prompting. Different types of prompts are explored and we choose results that show the best performance. Details of prompts can be found in Appendix~\ref{apx_c}.

% \paragraph{Encoder-Decoder Event Extractor}
% Given that deploying LLMs require expensive hard-ware and computation power, we also explore the method of training a small-scale event extractor to extract the events and associated time information. The extractor takes input the dialogue history and outputs the events that have been talked in the dialogue together with a the time duration and possible schedule of the events. We use the conversations and the associated events in~\dataset{} and fine-tune a T5 model~\cite{raffel2020exploring} as the extractor. We report the performance of the dialogue model with the event extractor in Appendix~\ref{apx_d}.

% \subsection{Model Training}
% We train all the models on ParlAI platform xxxxx.

% By modeling time, the most important feature we model is the relationship between the duration of progress events in previous sessions and the time gap between sessions. However, it is not clear what methods could best model such relationship. Therefore, we consider different methodologies for modeling time using~\dataset{} and explore the effectiveness of these methods.

% \subsection{Task Definition}
% We formulate the task of modeling time as a dialogue generation process. Let $u_i$ be one utterance of the conversation and $\mathcal{D}=\{u_0,u_1,...u_{n}\}$ be the dialogue history until turn $n$. $\Delta t$ is the time that has elapsed since $u_n$. Our task can be represented as generating the response $Y$ by:
% \begin{equation}
%     \hat{Y} = argmax\,P(Y|\mathcal{D},\Delta t)
% \end{equation}


% \subsection{Fine-Tuning without Time Annotations}
% We first fine-tune existing dialogue models on~\dataset{}, which will be the baseline systems in our final evaluation.

% \paragraph{MSC} This is the 2.7B encoder-decoder Transformer Blenderbot~\cite{roller-etal-2021-recipes} model fine-tuned on the MSC dataset. 
% We use this model as an initial pre-trianed model and further fine-tune it on \dataset{} to compare the performance. The model is extended to receive larger input (from 128 to 1024) to encode longer dialogue history.

% \paragraph{MSC RAG}
% To better deal with large scale of text, \citeauthor{xu-etal-2022-beyond} (\citeyear{xu-etal-2022-beyond}) used RAG (Retrieval-Augmented Generation)~\cite{lewis2020retrieval} models to store the dialogue history and enhance the memory. We follow this approach and fine-tune the MSC-RAG 2.7B model on \dataset{}. 

% \paragraph{SumMem-MSC RAG}
% To improve the efficiency of the RAG model, \citeauthor{xu-etal-2022-beyond} (\citeyear{xu-etal-2022-beyond}) alternatively summarize the dialogue history with an encoder-decoder summarizer and and store only summaries in the documents of the RAG model. Similarly, we use the same summarizer model to generate summaries and continue to train the model on \dataset{}.

% \subsection{Fine-Tuning with Time Annotations}
% \label{sec:model_time}
% Two important features we want to model are the duration of progress events in the previous sessions and the time gap between sessions. 
% We do this by first extracting the events with their associated duration and add such features to different models accordingly.

% \paragraph{Event extraction and duration annotation}
% With the data in \dataset{}, an encoder-decoder event extraction model that takes as input the history of previous sessions and outputs the event description and its duration is trained. 
% With this extraction model, we generate the possible events and their associated duration.

% \paragraph{Training with time annotations}
% For BST model, we simply concatenate the duration of events and the time gaps to the user inputs. For instance, the user input, ``I'm currently writing a conference paper.'' becomes ``I'm currently writing a conference paper. <writing a conference paper: 3 months> <gap: 3 hours>''. 
% For the RAG model, we follow the method proposed by ~\citeauthor{xu-etal-2022-beyond} and store the duration of the pre-defined progress events and the time gap between sessions in the documents.

% \subsection{Prompting LLMs}
% \label{sec:model_llm}
% During the collection of \dataset{}, we utilizes LLMs (ChatGPT). And that indicates that such LLMs potentially have perception of time. 
% It is necessary to explore how such LLMs could leverage the perception of time in conversation generation. Therefore, we also add the the conversations generated through prompting by different LLMs into comparison.

% \paragraph{ChatGPT}
% ChatGPT~\footnote{\url{https://openai.com/blog/chatgpt}} is a model trained using the Reinforcement Learning from Human Feedback (RLHF)~\cite{ouyang2022training} approach and shows state-of-the-art in a variety of NLP tasks.

% \paragraph{FLAN-T5}
% FLAN-T5~\cite{chung2022scaling} is the model fine-tuned on T5 model~\cite{raffel2020exploring} with instruct-tuning. It achieves strong few-shot performance when comparing to much larger models event with a smaller scale.

% \paragraph{LLaMA}
% LLaMA~\cite{touvron2023llama} is an open-source language model this is trained similar as ChatGPT. It is able to outperform GPT-3 175B event with only 13B parameters. 

% The performance of LLMs could significantly vary with different prompts and it is impossible to enumerate all types of prompts. In this work, we provide 5 different types of prompts that vary in template patterns~\cite{schick-schutze-2021-exploiting}, instance orders~\cite{lu-etal-2022-fantastically}, instruction descriptions~\cite{mishra-etal-2022-reframing} and add the best performance of each model into final comparison though the prompts for each model might be different. Details of the prompts can be found in Appendix C.

% \subsection{Dialogue Model + Prompting}
% Given that our dataset contains only limited pre-defined events, the event extraction model we use in Section~\ref{sec:model_time} might not perform well on arbitrary user inputs with random events. We further utilize the LLMs mentioned in Secion~\ref{sec:model_llm} to extract events and estimate the associated duration through prompting. This is done in a few-shot style, where several instances with their time annotations are selected from \dataset{} and ask LLMs to generate time annotations for arbitrary user inputs. 

% \input{Tables/fine_tune}


% Like in MSC, \dataset{} also contains multi-session conversations. Therefore, we also use the RAG (Retrieval-Augmented Generation)~\cite{lewis2020retrieval} approach to model time perception. However, to show the effectivess of \dataset{}, instead of training raw RAG models, we directly fine-tune the models proposed in~\cite{xu-etal-2022-beyond} on \dataset{}. This includes the the SumMem-MSC RAG and SumMem FiD-RAG model.

% \input{Tables/prompt}
% \paragraph{Duration of event and time gap between sessions}
% Two important features we want to model are the duration of progress events in the previous sessions and the time gap between sessions.
% For BST model, we simply concatenate the duration of events and the time gaps to the user inputs to provide such information. For instance, the user input, ``I'm currently writing a conference paper.'', the full input will become ``I'm currently writing a conference paper. <writing a conference paper: 3 months> <gap: 3 hours>''. In the RAG model, we follow the method proposed by ~\citeauthor{xu-etal-2022-beyond} and store the duration of the pre-defined progress events and the time gap between sessions in the documents.

% \paragraph{Event extraction and duration annotation} 
% Conversations in \dataset{} are collected based on the events that have been pre-defined.  Although we attempt to include various events with different duration in \dataset{}, it is impossible to include every possible event in the dataset and the model may receive events that are not pre-defined. It is necessary to automatically generate the schedules for such arbitrary events at inference time. To do that, we propose to extract the events and generate the schedules by large-scale language models (LLM) through prompting.

% The prompting procedure we present in this work has two rounds. In the first round, we provide LLM the dialogue history and extract the possible progress events. Table~\ref{tab:prompt} shows the prompt used for this round, where the instances are selected from \dataset{}, covering progress events with different duration. A sample response generated by the LLM could be ``writing a paper''. In the second round, we simply prompt the LLM to estimate the duration of each extracted progress event by inputting `Estimate roughly how long will it take to finish the following event: <extracted event>`. And we expect a time duration description of ``It takes about 3 months.'' from the LLM. In this work, we collect such duration annotations from GPT-3 davinci~\cite{brown2020language}.


==> trash/related.tex <==
% ======================= Qiang ============================== %
% \paragraph{Pragmatics Theory of Communication}
% Our work is greatly motivated by the pragmatics theory of communication. 
% ~\citeauthor{grice1975logic} (\citeyear{grice1975logic}) first proposed the cooperative principle (Gricean maxims, including quality, quantity, relevance and manner) to describe how people could have effective and informative conversations. ~\citeauthor{leech2016principles} (\citeyear{leech2016principles}) criticized that the Gricean maxims vagueness and proposed the politeness theory introducing the politeness maxims. 
% Apart from research in psychology, there are several works in NLP attempting to apply the pragmatics theory. For instance, some works show that ignoring social factors prevents applications from reaching human-level communications~\cite{hovy-yang-2021-importance}. There are also works build dialogue dataset with a focus of implicature~\cite{zheng-etal-2021-grice}. In our work, we claim that time is an important part of such social factors when providing effective conversations.

% Our work is primarily motivated by the cooperative principle (Gricean maxims) of communication, which was first introduced by~\citeauthor{grice1975logic} (\citeyear{grice1975logic}) to describe the mechanism of having effective conversations. Later works have been using the cooperative principle to evaluate conversations of both human-human~\cite{eskritt2008preschoolers,kleinke2010speaker} and human-computer~\cite{lan2020pone,langevin2021heuristic}. To better describe the quality of the follow-up questions asked by artificial agents, ~\citeauthor{ge2022should} (\citeyear{ge2022should}) proposed Gricean Scores that includes relevance, informativeness, truthfulness, clarity and coherence. Our work follows this line of works in terms of evaluating the information gain of the utterances generated by the model. The difference is that we specifically look into how the perception of time could affect the information gain.

% ======================= ChatGPT ============================== %
% Our work is primarily motivated by the pragmatic theory of communication. 
% The cooperative principle (Gricean maxims), which includes the principles of quality, quantity, relevance, and manner, was first introduced by \citeauthor{grice1975logic} (\citeyear{grice1975logic}) to explain how people can have informative and effective conversations. 
% However, the vagueness of the Gricean maxims has been criticized, and \citeauthor{leech2016principles} (\citeyear{leech2016principles}) proposed the politeness theory, which introduced the politeness maxims. 
% In addition to research in psychology, several works in natural language processing have attempted to apply the pragmatics theory. 
% For example, some studies have shown that ignoring social factors prevents applications from achieving human-like communication~\cite{hovy-yang-2021-importance}. 
% Other works have constructed dialogue datasets focusing on implicature~\cite{zheng-etal-2021-grice}. 
% Our work extends this line of research by arguing that time perception is an important aspect of social factors that contribute to effective conversations.

% ======================= Qiang ============================== %
% \paragraph{Long-term Dialogue Model}
% We build dialogue models based on previous works on multi-session long-term dialogue systems. 
% \citeauthor{xu-etal-2022-beyond} (\citeyear{xu-etal-2022-beyond}) first proposed the task of modeling multi-session conversations and released the Multi-Session Chat (MSC) dataset.
% MSC also claims that the main challenge in modeling multi-session conversations is the limited maximum input length in existing dialogue models.
% Therefore, MSC provides short summaries of previous sessions which will be encoded as context rather than the raw dialogue history. 
% Another work targeting at this issue is HAHT~\cite{zhang-etal-2022-history}, in which different sessions will be encoded independently into vectors and aggregated as is done in attention mechanism. 
% Apart from that, there are also other works modeling different external attributes such as persona~\cite{xu-etal-2022-long} in long-term conversations.
% Unlike this previous works, ours studies the effectiveness of an important but ignored aspect of perception of time in long-term conversations.

% ======================= ChatGPT ============================== %
% ======================= Qiang ============================== %
% Our work is also related to topic-aware dialogue models that select appropriate topics for further conversations. ~\citeauthor{somasundaran2020two} (\citeyear{somasundaran2020two}) selects topics based on extracted topic segments. Later work also extends this method to capture topic segments at a global discourse-level~\cite{xu2021topic}. There are also works that tries to detect and follow the topic-shifts~\cite{xie2021tiage} or trigger context-controlled topic transitions~\cite{ling2021context} in the conversation. These works are able to capture the topic transition and select appropriate topics based on the word-level or sentence-level semantics in the dialogue history. Our work differs from these works in that we introduce explicit external time perception, which does not exist in the dialogue context as a factor for selecting topic. 
